Finding large balanced subgraphs in signed networks

Signed networks are graphs whose edges are labelled with either a positive or a negative sign, and can be used to capture nuances in interactions that are missed by their unsigned counterparts. The concept of balance in signed graph theory determines whether a network can be partitioned into two perfectly opposing subsets, and is therefore useful for modelling phenomena such as the existence of polarized communities in social networks. While determining whether a graph is balanced is easy, finding a large balanced subgraph is hard. The few heuristics available in the literature for this purpose are either ineffective or non-scalable. In this paper we propose an efficient algorithm for finding large balanced subgraphs in signed networks. The algorithm relies on signed spectral theory and a novel bound for perturbations of the graph Laplacian. In a wide variety of experiments on real-world data we show that our algorithm can find balanced subgraphs much larger than those detected by existing methods, and in addition, it is faster. We test its scalability on graphs of up to 34 million edges.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> notes.tex <==
\subsection{Algorithm overview}
\begin{itemize}
\item Compute the upper bound for all vertices
\item Iterate: find minimum and remove all dependent vertices, until none left. Put all found minima in set $S$
\item For each $v$ in $S$, fetch eigenvectors of perturbation, multiply by $V$ and look for new $\lambda$.
\item To find new $\lambda$, use Krylov subspace method to solve linear system of eigenvalue 1.
\item Cut off where desired.
\end{itemize}

\subsection{Considerations}
\begin{itemize}
\item The eigenvectors of a star are always the same (I think: prove). They only chage with degree, so no need to compute them. This should be easy to prove once we have the spectrum.
\item In addition to being always the same, they are sparse (as sparse as the degree of the vertex.)
\item To find the new eigenvalue we only need to set $\lambda$ so that $U^T(\lambda-\Lambda)^{-1}U$ has an eigenvalue equal to 1. Each bisection step is expensive. In our favor we can argue that the matrices involved are usually small. We can support this with the experiments.
\item To do bisection efficiently we should prove that $\lambda$ decreases with each added independent vertex.
\item Can we just sum the reduction of eigenvalue of each independent vertex to get a good bound? How does this compare to the actual computation of the new eigenvalue?
\item A way to find zeros fast can be to use one of LU, Cholesky or QR and look for a zero in the diagonal.
\item Since the algorithm will no doubt be less efficient that simple spectral partitioning, we can also compare if the upper bound provides a better ranking than the Laplacian eigenvector.
\item We need to decide the threshold at which we consider a subgraph balanced, because the minimum eigenvalue is estimated.
\item One thing to highlight is that our algorithm gradually reduces imbalance, so we can trade off size and density for balance.
\item Something that happens is that we tend to find large exclusively positive communities. This is not bad. Traditional community detection algorithms will detect dense subgraphs, but can't consider edge signs.
\item Try to think of illustrative examples:
  \begin{itemize}
  \item To show our algorithm is correct in some sense where others aren't
  \item To show our algorithm tends to remove sparse elements (e.g. a balanced triangle that is connected to only one vertex)
  \item To show why we must consider independent vertices
  \end{itemize}
\end{itemize}



==> problem.tex <==
Our main goal is to find insightful relationships between variables in data. For instance, consider Marta's survey data. It is comprised of respondents' answers to questions like ``How much do you trust institutions?'' or ``How strongly do you support LGBT activism?''. It is to be expected that some relationships will arise. For instance, one would expect attitudes towards LGBT activism to correlate strongly with religious feelings. We also want to consider higher-order relationships. For instance, it might be the case that all variables related to immigratioin policies are well predicted based on attitudes towards LGBT activism in combination with trust in institutions. In a nutshell, we look for multiple correlations, or subsets of variables that can be explained by a small number of factors (and ideally, these factors can be expressed in terms of actual variables).

When aiming for interpretable low-rank approximations, subset selection methods are often regarded as a good choice. In particular, given a matrix $A \in \mathbb R^{m\times n}$ and a target rank $k \in \mathbb N$, one tries to minimize the following function over $C$:
\[
\|A-CC^+A\|_F^2,
\]
where $C$ is comprised of a subset of $k$ columns of $A$. In words, we search for the columns of $A$ that are the most representative of the full matrix. Since we express our data in terms of a small number of our original variables, this approach is often deemed adequate for interpretability and insight.

However, this method can still fail in this regard, due to various reasons:
\begin{itemize}
\item The solution produces a $k\times n$ linear model, which can be difficult to make sense of for relatively large $k$ and $n$.
\item It is global, while some insightful relationships between variables might be local. An example to illustrate this is given below.
\end{itemize}

As an example to illustrate the second point above, we propose the following. Consider a matrix $A=\left ( B ~ C \right )$ (the concatenation of $B$ and $C$), with $\|C\|\gg\|B\|$ and $\rank (C)\gg\rank(B)\approx 1$. An algorithm to approximately factorize $A$ with an approximation of rank $k\leq\rank(C)$ will generally focus on recovering $\|C\|$, and will fail to identify the rank-$1$ cluster $B$. That is, while it is possible to approximate the columns of $B$ with a single one of them, which might be a useful finding to practitioners, the column subset selection algorithm might miss this fact.

Of course, we would also like to handle cases where the rank of $B$ is small but larger than $1$.

To alleviate the shortcomings described above, we propose the following approach.

Our method is based on two building-blocks: close-to-rank-one (CRO) clustering \cite{kim2007method} and column subset selection (CSS).

\subsection{CRO clustering}
Given a matrix $A$, its CRO is defined as
\[
\rho(A)=\frac{\|A\|_2^2}{\|A\|_F^2}.
\]
That is, it determines how close it is to being rank-$1$. CRO clustering creates column clusters to maximize the sum of CRO's. An algorithm for CRO clustering can be defined as follows.


Input: $m\times n$ matrix $A$, number of clusters $k$.
\begin{enumerate}
\item Initialize $n$ clusters, each comprised of a distinct column of $A$.
\item \label{cro_stepone} Consider all pairs of clusters and compute their CRO.
\item Merge the cluster pair with largest CRO.
\item Repeat from step \ref{cro_stepone} until $k$ clusters are left.
\end{enumerate}

  
\subsection{Column subset selection}
Consider a column-subset $B_i$ of $A$ with $1-\rho(B_i)\leq \epsilon$. This means $\|B_i\|_F^2-\sigma_1^2(B_i) \leq \epsilon \|B_i\|_F^2$. If we cluster columns so that every subset $B_i$ satisfies this inequality, we can then perform Guruswami-Sinop CSS \cite{guruswami2012optimal} and obtain
\[
\|B_i-C_iC_i^+B_i\|_F^2 \leq  \left(1+1/r\right) \epsilon\|B_i\|_F^2.
\]
This suggests the following algorithm:

\begin{figure}
Input: $m\times n$ matrix $A$, loss threshold $\epsilon$.
\begin{enumerate}
\item Initialize $n$ clusters, each comprised of a distinct column of $A$.
\item \label{cro_stepone} Consider all pairs of clusters and compute their CRO.
\item Merge the cluster pair with largest CRO, provided it is above $1-\epsilon$.
\item Repeat from step \ref{cro_stepone} until no cluster with CRO above  $1-\epsilon$ can be formed.
\end{enumerate}
\caption{Clustered CSS Algorithm}
\label{alg:CCSS}
\end{figure}

This means that we can set a loss threshold $\epsilon$ and find clusters of well-factored variables. ``Well-factored'' means that we can choose a subset of $r$ variables in each cluster that represent the whole cluster with a loss of at most $\left(1+1/r\right)\epsilon$.


\subsection{Problem formulations}
\begin{problem}
\label{prob:atleast}
  Given a matrix $A$ and a threshold $0<\tau\leq 1$, determine whether there is a subset of at least 2 columns with CRO at least $\tau$.
\end{problem}

\begin{problem}
\label{prob:max_cro}
  Given a matrix $A$ and a threshold $0<\tau\leq 1$, find the largest CRO attainable by column subset of $A$.
\end{problem}

\begin{problem}
\label{prob:best_subset}
  Given a matrix $A$ and a threshold $0<\tau\leq 1$, find the largest column subset with CRO at least $\tau$.
\end{problem}

\begin{problem}
\label{prob:largest_subset}
  Given a matrix $A$ and a number $k\in \mathbb N$, find the column subset of size $k$ with largest CRO.
\end{problem}

\subsection{Normalized CRO (No-CRO)}
CRO clustering has a pitfall. If $\|u\| \ll \|C\|$ then $\rho(\{u\} \cup C)\approx 1$. In practice, one tipically wants an algorithm that is not sensitive to scale. For this reason, we consider a family of CRO-based problem instances where we assume $\|u\|=1$ for all columns $u$ of the input matrix. We refer to this problem as Normalized CRO (No-CRO).

